Compressing Convolutional Neural Networks

Convolutional neural networks (CNN) are increasingly used in many areas of computer vision. They are particularly attractive because of their ability to "absorb" great quantities of labeled data through millions of parameters. However, as model sizes increase, so do the storage and memory requirements of the classifiers. We present a novel network architecture, Frequency-Sensitive Hashed Nets (FreshNets), which exploits inherent redundancy in both convolutional layers and fully-connected layers of a deep learning model, leading to dramatic savings in memory and storage consumption. Based on the key observation that the weights of learned convolutional filters are typically smooth and low-frequency, we first convert filter weights to the frequency domain with a discrete cosine transform (DCT) and use a low-cost hash function to randomly group frequency parameters into hash buckets. All parameters assigned the same hash bucket share a single value learned with standard back-propagation. To further reduce model size we allocate fewer hash buckets to high-frequency components, which are generally less important. We evaluate FreshNets on eight data sets, and show that it leads to drastically better compressed performance than several relevant baselines.

==> content/notation.tex <==
%!TEX root=../nips2015.tex


\section{Notation}
Throughout this paper we type vectors in bold ($\bx$), scalars in regular ($C$ or $b$) and matrices in capital bold ($\mathbf{X}$). Specific entries in vectors or matrices are scalars and follow the corresponding convention, $i.e.$ the $i^{th}$ dimension of vector $\mathbf{x}$ is $x_i$ and the $(i,j)^{th}$ entry of matrix $\mathbf{V}$ is $V_{ij}$. 




% \paragraph{Feed Forward Neural Networks.}
% We define the forward propagation of the $\ell^{th}$ layer in a neural networks as,
% \begin{equation}
% 	a^{\ell+1}_i = f(z^{\ell+1}_i),  ~~~\text{where}~~ z^{\ell+1}_i = \sum_{j=0}^{n^\ell} V_{ij}^\ell a^\ell_j,\label{eq.output_std}
% \end{equation}
% where $\bV^\ell$ is the (virtual) weight matrix in the $\ell^{th}$ layer. The vectors $\bz^\ell, \ba^\ell\!\in\!{\cal R}^{n^\ell}$  denote the activation units before and after transformation through the transition function $f(\cdot)$.
% Typical activation functions are rectifier linear unit (ReLU)~\cite{nair2010rectified}, sigmoid or tanh~\cite{lecun2012efficient}.




==> content/table_nlcf6.tex <==
%!TEX root=../nips2015.tex

% May 27 result
\begin{table}
\centering \small
\begin{tabular}{r|c|ccc}
 & \textbf{CNN} & \textbf{LRD} & \textbf{HashedNets} & \textbf{\abbrevtable{}} \\
\hline
\data{cifar10}  & $14.37$ & $34.35$ & $43.08$ & \boldBlue{30.79} \\
\data{cifar100} & $33.76$ & $66.44$ & $67.06$ & \boldBlue{62.33} \\
\data{svhn}     & $3.69$  & $22.32$ & $23.31$ & \boldBlue{18.37} \\
\data{mnist-07} & $0.85$  & $1.95$  & $1.77$  & \boldBlue{1.24}  \\
\data{rot }     & $3.32$  & $9.90$  & $10.10$ & \boldBlue{6.60}  \\
\data{bg-rot}   & $11.28$ & $35.64$ & $32.40$ & \boldBlue{27.91} \\
\data{bg-rand}  & $1.77$  & $4.57$  & $5.10$  & \boldBlue{3.62}  \\
\data{bg-img}   & $2.38$  & $7.23$  & \boldBlue{6.68}  & $8.04$  \\
\end{tabular}
\caption{Test error rates (in $\%$) with compression factor $1/64$. (The fully connected layer is compressed to $1/64$ in all methods using HashedNets. No compression was applied to the convolutional layers of CNN.)}
\label{table:nlcf6}
\end{table}

% May 26 result
% \begin{table}
% \centering
% \begin{tabular}{c|c|ccc}
%  & \textbf{CNN} & \textbf{LRD} & \textbf{HashedNets} & \textbf{\abbrev{}} \\
% \hline
% \data{cifar10}  & 14.37 & 34.35 & 43.08 & \boldBlue{30.79} \\
% \data{cifar100} & 33.76 & 66.44 & 67.06 & \boldBlue{62.33} \\
% \data{svhn}     & 3.69 & 22.32 & 23.31 & \boldBlue{18.37} \\
% \data{mnist-07} & 0.85 & 1.95 & 1.77 & \boldBlue{1.24} \\
% \data{rot }     & - & - & 10.10 & \boldBlue{6.60} \\
% \data{bg-rot}   & 11.28 & 35.64 & 32.40 & \boldBlue{27.91} \\
% \data{bg-rand}  & - & 4.57 & 5.10 & \boldBlue{3.62} \\
% \data{bg-img}   & - & \boldBlue{-} & - & - \\
% \end{tabular}
% \caption{Compression factor = $1/64$. (The fully connected layer is compressed to $1/64$ in all methods using HashedNets. No compression was applied to the convolutional layers of CNN.)}
% \label{table:nlcf6}
% \end{table}


% \begin{table}
% \centering
% \begin{tabular}{|c||c|c|c|c|}
% \hline
%  & CNN (top hashed) & LRD & HashedNet & dct-HashedNet \\
% \hline
% CIFAR-10 & 14.37 & 34.35 & 43.08 & \boldBlue{30.79} \\
% \hline
% CIFAR-100 & 33.76 & 66.44 & 67.06 & \boldBlue{62.33} \\
% \hline
% SVHN & 3.69 & 22.32 & 23.31 & \boldBlue{18.37} \\
% \hline
% MNIST-ICML07 & - & \boldBlue{-} & - & - \\
% \hline
% ROT & - & - & 10.10 & \boldBlue{6.60} \\
% \hline
% BG-RAND & - & - & 5.10 & \boldBlue{3.62} \\
% \hline
% \end{tabular}
% \caption{Compression factor = 1/64}
% \label{table:nlcf6}
% \end{table}


% \begin{table}[h]
% 	\centering
% 	\begin{tabular}{|c|c|c|c|c|c|c|}
% 	\hline
% 	 & CNN & dropFilt & dropFreq & LRD & HashNet & 4Net \\
% 	\hline
% 	CIFAR-10 & 14.37 & - & - & 34.35 & 43.08 & \boldBlue{30.79} \\
% 	\hline
% 	CIFAR-100 & - & - & - & 66.44 & 67.06 & \boldBlue{62.33} \\
% 	\hline
% 	SVHN & - & - & - & 22.32 & 23.31 & \boldBlue{18.37} \\
% 	\hline
% 	\end{tabular}
% 	\caption{NLCF = 6}
% 	\label{table:nlcf6}
% \end{table}



